Learning the Optimal Stopping for Early Classification within Finite Horizons via Sequential Probability Ratio Test

Time-sensitive machine learning benefits from Sequential Probability Ratio Test (SPRT), which provides an optimal stopping time for early classification of time series. However, in finite horizon scenarios, where input lengths are finite, determining the optimal stopping rule becomes computationally intensive due to the need for backward induction, limiting practical applicability. We thus introduce FIRMBOUND, an SPRT-based framework that efficiently estimates the solution to backward induction from training data, bridging the gap between optimal stopping theory and real-world deployment. It employs density ratio estimation and convex function learning to provide statistically consistent estimators for sufficient statistic and conditional expectation, both essential for solving backward induction; consequently, FIRMBOUND minimizes Bayes risk to reach optimality. Additionally, we present a faster alternative using Gaussian process regression, which significantly reduces training time while retaining low deployment overhead, albeit with potential compromise in statistical consistency. Experiments across independent and identically distributed (i.i.d.), non-i.i.d., binary, multiclass, synthetic, and real-world datasets show that FIRMBOUND achieves optimalities in the sense of Bayes risk and speed-accuracy tradeoff. Furthermore, it advances the tradeoff boundary toward optimality when possible and reduces decision-time variance, ensuring reliable decision-making. Code is publicly available at https://github.com/Akinori-F-Ebihara/FIRMBOUND

==> Convexity.tex <==
\section{On the Concavity of the Conditional Expectation}\label{app:concavity}
We review the concave property of the conditional expectation based on the discussion in~\cite{TartarBook}. To prove concavity, we first need to review (1) in what sense SPRT is optimal within the finite horizon, (2) why computing the backward induction leads to minimizing AAPR, thereby proving that (3) the conditional expectation is concave.

\subsection{SPRT Under Finite horizon is the Optimal Bayes Risk Minimizer}
% In estimation and decision theory, a Bayes estimator or a Bayes action minimizes the posterior expected value of a loss function (i.e., Bayes risk, or AAPR), which is also known as the posterior expected loss. In other words, it maximizes the posterior expectation of a utility function. Another approach in Bayesian statistics is to formulate an estimator using maximum a posteriori estimation. Formally:
In estimation and decision theory, a Bayes estimator or Bayes action minimizes the posterior expected value of a loss function, also known as the Bayes risk or AAPR, which is equivalent to minimizing the posterior expected loss. 
% In other words, it aims to maximize the posterior expectation of a utility function. 
Another approach in Bayesian statistics involves formulating an estimator using maximum a posteriori estimation. Formally:
\begin{definition}[\textbf{Bayes risk.}]\label{def:bayes_risk}
Consider an unknown parameter $\theta$ with a known prior distribution $\pi$. Define ${\hat{\theta }}={\hat{\theta }}(x)$ as an estimator of $\theta$, based on measurements $x$, and let $L(\theta, {\hat{\theta }})$ represent a loss function. The Bayes risk of ${\hat{\theta }}$ is defined as $E_{\pi }[L(\theta, {\hat{\theta }})]$, where the expectation is taken over the probability distribution of $\theta$. This quantifies the estimator's risk as a function of ${\hat{\theta }}$. An estimator ${\hat{\theta }}$ is termed a Bayes estimator if it minimizes the Bayes risk among all possible estimators. Equivalently, an estimator that minimizes the posterior expected loss $E[L(\theta, {\hat{\theta }}) \mid x]$ for each $x$ also minimizes the Bayes risk, thus qualifying as a Bayes estimator.
\end{definition}

Bayesian decision rule, or stopping rule, is formulated as follows:

% TartarBook p.66-67
\begin{definition}[\textbf{Bayesian decision rule.}]\label{def:bayesian_decision_rule}
An optimal Bayesian decision rule, or optimal sequential decision rule, $\delta^*$ is defined as the rule that minimizes the AAPR, or expected risk, denoted by $\rho(\delta) := \mathbb{E}_{X^{(1,T)}}[L_\tau (\theta_\tau, d_T(X^{(1,T)}),X^{(1,T)})]$ Note that $\rho(\delta)$ is the Bayes risk according to (1) (denoted by $E_{\pi }(L(\theta ,{\hat{\theta }}))$ above). Thus, the task $\min_T \rho(\delta)$ with $\delta=(d, \tau)$ is a sequential Bayes risk minimization problem.
\end{definition}

Where $\theta$ can be regarded as a hypothesis to be tested with SPRT. Note that SPRT is the optimal algorithm under the framework of Def.~\ref{def:bayesian_decision_rule}.

It is shown that finding an optimal Bayesian decision rule $\delta^*$ reduces to finding an optimal stopping rule $\tau^*$ that minimizes AAPR $\rho(d^*, \tau)$ because the optimal \textit{terminal rule} $d^*$ does not depend on the \textit{stopping rule} $\tau$.

Furthermore, it is shown that
\begin{equation} \label{eq: def of AVR}
    \rho(d^*, \tau) = \mathbb{E}_{X^{(1,T)}}[R^*_t(X^{(1,T)})],
\end{equation}
where 
\begin{align} 
    R_t^*(X^{(1,t)}) :=& R_t(X^{(1,Tt}, d^*(X^{(1,t)})) \nonumber \\
    =& \inf_d R_t(X^{(1,t)}, d(X^{(1,t)}))    
\end{align}
is the minimal APR, and 
\begin{align}
    R_t(X^{(1,t)}, d^*(X^{(1,t)})) :=& \mathbb{E}[L_m(\theta_n, d(X^{(1,t)}), X^{(1,t)}) | X^{(1,t)}] \nonumber\\ 
    =& \int d\theta_n L_t(\theta_t, d(X^{(1,t)}), X^{(1,t)}) \pi_t(\theta_t|X^{(1,t)})    \label{eq: def of APR}
\end{align}

is the APR.
Therefore, our task $\min_T \rho(\delta)$ with Eq.~\ref{eq: def of AVR} is equivalent to finding an optimal stopping rule $\tau^*$ that minimizes the AAPR.

\paragraph{Remark.} Bayes risk minimization problem, which is equivalent to minimizing AAPR, reduces to $\inf_T \rho(d^*, T) = \inf_\tau \mathbb{E}^\pi[\min(L_1\pi_\tau, L_0(1-\pi_\tau)) + c\tau]$ (equivalent to Eq.~\ref{eq: def of AVR}), and the optimal algorithm of which is proven to be SPRT~\citep{TartarBook}. Therefore, SPRT is the optimal sequential decision rule of a sequential Bayes risk minimization problem. More details can be found in~\cite{TartarBook}.

\subsection{Computing the Backward Induction Eq.~\ref{eq:backward_induction} Minimizes AAPR}
% At a glance, it is not very intuitive why SPRT achieves Bayes optimality under finite horizon by solving the backward induction equation. Consider a general scheme, where $\Psi \ \{\Psi_t\}_{t\geq 1}$ be a sequence of random variables (rewards or gains, not risks) on the filtered probability space $(\Omega, \mathscr{F}, \{\mathscr{F}_t\}, P)$ adapted to the filtration $\{\mathscr{F}_t\}_{t \geq 1}$, where $\{\mathscr{F}_t\}$ is an increasing dequence of sigma-algebras. The sigma-algebra $\mathscr{F}$ is cumulative information that we obtain up to time $t$. Let $W_t$, $t=1,...,T$ be optimal rewards when information $\mathscr{F}$ is available. Then the following theorem gives the exact result under the finite horizon.
At first glance, it may not seem intuitive why SPRT achieves Bayes optimality under a finite horizon by solving the backward induction equation. Consider a general scheme where $\Psi = \{\Psi_t\}_{t \geq 1}$ is a sequence of random variables (rewards or gains, not risks) on the filtered probability space $(\Omega, \mathscr{F}, \{\mathscr{F}_t\}, P)$ adapted to the filtration $\{\mathscr{F}_t\}_{t \geq 1}$, an increasing sequence of sigma-algebras. Here, $\mathscr{F}_t$ represents the cumulative information available up to time $t$. Let $W_t$ for $t=1, \ldots, T$ be the optimal rewards when information from $\mathscr{F}_t$ is available. The following theorem provides the exact result under the finite horizon.

% TartarBook p.68, Thm. 2.7.1
\begin{theorem}\label{thm:finite_horizon_optimal_stopping}
(Finite horizon optimal stopping~\citep{TartarBook}.) Let the sequence \(\{W^t\}_{1 \leq t \leq T}\) be defined by the recursion
\begin{equation}
W_t = \max \{\Psi_t, E[W_{t+1} \mid \mathscr{F}_t]\}, \quad t = T-1, T-2, \ldots, 1,
\end{equation}
and let the stopping time $\tau$ be defined as in
\begin{equation}
\tau = \min \{1 \leq t \leq T : \Psi_t = W^t\}.
\end{equation}
Assume that the sequence \(\{\Psi_t\}_{1 \leq t \leq T}\) is integrable. Then $\tau$ is the optimal stopping rule in the class of $T$-truncated stopping rules, i.e.,
\begin{equation}
V_T = \sup_{\tau} E[\Psi_\tau] = E[\Psi_\tau^*]
\end{equation}
and
\begin{equation}\label{eq:finite_horizon_optimal_stopping}
    V_T = \mathbb{E}[W_1] \, ,
\end{equation}
where $V_T$ is the optimal gains in $T$-truncated problem. 
\end{theorem}
The proof is provided in~\cite{TartarBook}. 

Eq.~\ref{eq:finite_horizon_optimal_stopping} indicates that $W_1$ serves as a comprehensive decision metric that encapsulates the entire strategy for sequential decision-making, ensuring that the initial setup already aims for the overall best outcome by considering all future possibilities. In other words, the first step is made with full knowledge of the optimal outcomes of all subsequent decisions. This does not imply that the first step alone is sufficient to optimize the entire sequence in isolation, but rather, the calculation of Eq.~\ref{eq:finite_horizon_optimal_stopping} inherently includes optimal decision-making at each subsequent step.

By applying Thm.~\ref{thm:finite_horizon_optimal_stopping}, we obtain the following general result for Bayesian decision-making under a finite horizon.
% TartarBook p.72
\begin{theorem}[Solution of backward induction minimizes Bayes risk~\citep{TartarBook}.]\label{thm:optimal_BayesRisk}
    Assume that in the sets of terminal decisions $\mathcal{D}_n$ ($n = 1,2,\dots,T$), there exist the elements $u_t^* := d^*(X^{(1,t)})$ for which the infimums $R_t(X^{(1,t)}, u_t^*) = \inf_{u_t \in \mathcal{D}_t}R_t(X^{(1,n)}, u_t)$ are attained, where $R_t$ is the APR defined in Eq.~\ref{eq: def of APR}.    
    Let the sequence $\{ R_t \}_{n=1}^T$ be defined by the backward induction equation
    \begin{equation} \label{eq: BIE}
        R_T^{\mathrm{min}} = R_T^{\rm st}, \quad 
        R_t^{\mathrm{min}} = \min\{ R_t^\mathrm{st}, \mathbb{E}[R_{t+1}^{\rm min} | X^{(1,n)}] \}, \quad
        t = T-1, T-2, \dots, 1\, ,
    \end{equation}
    where $R_t^\mathrm{st} := R_t^*(X^{(1,T)})$ is the minimum APR of realization $X^{(1,T)}$.
    Then, the optimal Bayesian $T$-truncated rule exits and $R_1^{\rm min}$ gives the optimal Bayes risk: 
    \begin{equation} \label{eq:minimal_bayes_risk_is_expectation_at_the_first_step}
        \rho^* = \mathbb{E}[R_1^{\rm min}].
    \end{equation}{}
\end{theorem}

The Eq.~\ref{eq:minimal_bayes_risk_is_expectation_at_the_first_step} is exactly the final output of the backward equation that is computed from the $t=T$ horizon back to the first step. 
%Note that the discussion is unchanged by subtracting the linear sampling cost $ct$ to have $G_t^{\mathrm{min}} = R_t^{\mathrm{min}}-ct$.



\subsection{The Conditional Expectation Eq.~\ref{eq:continuation_risk} is a Concave Function}
Now, we are ready to review that the conditional expectation that appears in the backward induction is strictly a concave function:

\begin{theorem}\label{thm:concavity}
(Concavity of the conditional expectation~\citep{TartarBook}.) $G_t^{\mathrm{min}}(\pi)$ are concave functions of $\pi$ in $[0,1]$ for every $T \geq t$, including the nontruncated case $T = \infty$.
\end{theorem}
% \textbf{Lemma 3.2.2.} $G_N^\pi(\pi)$ are concave functions of $\pi$ in $[0,1]$ for every $N \geq n$, including the nontruncated case $N = \infty$.

\textbf{Proof.} To prove the first assertion it suffices to show that $G_1^{\mathrm{min}}(\pi)$ is concave for each $1 \leq T \leq \infty$. By Thm.~\ref{thm:optimal_BayesRisk}, $G_1^{\mathrm{min}}(\pi)$ is nothing but the minimum average Bayes risk:
\begin{equation}
    G_1^\pi(\pi) = \rho_1(\pi) = \inf_\tau \rho_T(\pi, \tau),
\end{equation}
where $\tau$ is the hitting time. Furthermore, $\rho_T(\pi, \tau)$ is linear in $\pi$. Indeed,
\begin{align}
    \rho_T(\pi, \tau) &= \mathbb{E}^\pi[\bar{L}(\theta, d^*) + c\tau] \nonumber \\
    &= \sum_k \pi_k \mathbb{E}_k[\bar{L}(\theta = k, d^* \neq k) + c\tau] \nonumber \\
    &= \sum_k \pi_k\bar{L}P_k(d^* \neq k) + \sum_k \pi_k c \mathbb{E}_k[\tau] 
    % &= \pi E_1[L(\theta = 1, d^*) + cT] + (1 - \pi) E_0[L(\theta = 0, d^* = 1) + cT].
\end{align}
Hence, for every $0 < \alpha < 1$, $\pi_1$ and $\pi_2$,
\begin{align}
G_1^{\mathrm{min}}(\alpha \pi_1 + (1 - \alpha) \pi_2) &= \inf_\tau \rho_T(\alpha \pi_1 + (1 - \alpha) \pi_2, \tau) \nonumber \\
&\geq \alpha \inf_\tau \rho_T(\pi_1, \tau) + (1 - \alpha) \inf_\tau \rho_T(\pi_2, \tau) \nonumber \\
&= \alpha G_0^{\mathrm{min}}(\pi_1) + (1 - \alpha) G_0^{\mathrm{min}}(\pi_2).
\end{align}
For $T = \infty$ the proof is identical. Therefore, we proved that $G_t^{\mathrm{min}}(\pi)$ is a concave function of $\pi$ for each $1 \leq T \leq \infty$.

Now,
\begin{equation}
% G_{n,1}^\pi(\pi_n) = c + E^T[G_{n+1}^\pi(\pi_{n+1}) | \pi_n],
\tilde{G}_t(\pi_t) = \mathbb{E}\left[
            {G}^{\mathrm{min}}_{t+1}(\pi_{t+1})    
            |\pi_{t})\right] + c
\end{equation}
where ${G}^{\mathrm{min}}_{t+1}$ is concave by the first assertion. It can be shown that the conditional expectation $\mathbb{E}\left[
            {G}^{\mathrm{min}}_{t+1}(\pi_{t+1})    
            |\pi_{t})\right]$ is also a concave function, so that both assertions of the lemma follow.



% \begin{theorem}\label{thm:finite_horizon_optimal_stopping}
% % \textbf{Thm. 2.7.1} (Finite horizon optimal stopping). 
% (Finite horizon optimal stopping) Let the sequence \(\{W^n\}_{1 \leq n \leq N}\) be defined by the recursion
% \[
% W^n = \max \{\Psi^n, E[W^{n+1} \mid \mathcal{F}_n]\}, \quad n = N-1, N-2, \ldots, 1,
% \]
% and let the stopping time \(T^*_N\) be defined as in
% \[
% T^*_N = \min \{1 \leq n \leq N : \Psi_n = W^n\}.
% \]
% Assume that the sequence \(\{\Psi^n\}_{1 \leq n \leq N}\) is integrable. Then \(T^*_N\) is the optimal stopping rule in the class of $N$-truncated stopping rules \(M^N\), i.e.,
% \[
% V_N = \sup_{\tau \in M^N} E[\Psi^\tau] = E[\Psi^{T^*_N}]
% \]
% and
% \[
% V_N = E[W^1].
% \]
% \end{theorem}

% \subsection*{Proof}

% Let \(W^N\) be given by the recursion 
% \[
% W^n = \max \{\Psi^n, E[W^{n+1} \mid \mathcal{F}_n]\},
% \]
% and let \(T^*_N\) be the stopping time defined in
% \[
% T^*_N = \min \{1 \leq n \leq N : \Psi_n = W^n\}.
% \]
% We now prove that for every \(n = 1, \ldots, N\),
% \[
% E[\Psi^{T^*_N} \mid \mathcal{F}_n] = W^n \geq E[\Psi^\tau \mid \mathcal{F}_n] \text{ for all } \tau \in M^N,
% \]
% which implies that
% \[
% E[\Psi^{T^*_N}] = E[W^1] \geq E[\Psi^\tau] \text{ for all } \tau \in M^N \text{ and all } n = 1, \ldots, N.
% \]
% Relations yield in particular the statement of the theorem setting \(n = 1\). For \(n = N\) the result holds trivially. The proof will be conducted by induction. Suppose 
% \[
% E[\Psi^{T^*_N} \mid \mathcal{F}_{n-1}] = E[W^n \mid \mathcal{F}_{n-1}] \geq E[\Psi^\tau \mid \mathcal{F}_{n-1}] \text{ for some } n \in \{1, \ldots, N\}.
% \]
% Let \(A_{n-1} \in \mathcal{F}_{n-1}\) be an arbitrary event and \(\tau_n = \max(T^*_N, n)\). We have
% \begin{align*}
% E[\Psi^{T^*_N} \mid A_{n-1}] & = E[\Psi^{\tau_n} \mid A_{n-1}] \\
% & = E[\Psi^{\tau_n} \mid A_{n-1}, \tau_n = n] + E[\Psi^{\tau_n} \mid A_{n-1}, \tau_n > n] \\
% & = E[\Psi_n \mid A_{n-1}, \tau_n = n] + E[\Psi_{n+1} \mid A_{n-1}, \tau_n > n] \\
% & = E[E[\Psi_n \mid \mathcal{F}_n] \mid A_{n-1}, \tau_n = n] + E[\Psi_{n+1} \mid A_{n-1}, \tau_n > n] \\
% & = E[\max(\Psi_{n-1}, E[W^n \mid \mathcal{F}_n]) \mid A_{n-1}] \\
% & = E[W^{n-1} \mid A_{n-1}].
% \end{align*}
% Since the event \(A_{n-1} \in \mathcal{F}_{n-1}\) is arbitrary, it follows that
% \[
% W^{n-1} = E[\Psi^{T^*_N} \mid \mathcal{F}_{n-1}],
% \]
% and the proof of the theorem is complete.

% \begin{theorem}\label{thm:optimal_BayesRisk}
% (Thm. 2.7.4 in~\cite{TartarBook}) Assume that in the sets of terminal decisions \(D_n\), \(n = 1, \ldots, T\), there exist the elements \(\mu_t\), \(t = 1, \ldots, T\) for which the infimums in Eq. \ref{eq:APR} are attained. 
% Suppose that \(\mathbb{E}[\max_{t \leq T} G^{st}_t] < \infty\), 
% Then, the optimal Bayesian risk is \(\rho^*_T = E[G^{\mathrm{min}}_1]\).
%     \begin{enumerate}
%         \item[(i)] Then the optimal Bayesian \(T\)-truncated rule exists and has the form \(\delta^* = (\delta^*_N, T^*_N)\), where \(T^*_T = \min\{1 \leq t \leq T : G^{\mathrm{min}}_t = \min_{1 \leq t \leq T} G^{\mathrm{min}}_t\}\), and \(\delta^*_n = \mu_n\) if \(T^*_N = n\).
%         \item[(ii)] The optimal Bayesian risk is \(\rho^*_T = E[G^{\mathrm{min}}_1]\).
%     \end{enumerate}
% \end{theorem}

% \textbf{Thm. 2.7.4.} Assume that in the sets of terminal decisions \(D_n\), \(n = 1, \ldots, N\), there exist the elements \(\mu_n\), \(n = 1, \ldots, N\) for which the infimums in (2.181) are attained. Let the sequence \(\{R^N_n\}_{n=1}^N\) be defined by the recursion (2.207). Suppose that \(E[\max_{n \leq N} R^N_n] < \infty\).

% \begin{enumerate}
%     \item[(i)] Then the optimal Bayesian \(N\)-truncated rule exists and has the form \(\delta^* = (\delta^*_N, T^*_N)\), where \(T^*_N = \min\{1 \leq n \leq N : R^N_n = \min_{1 \leq m \leq N} R^N_m\}\), and \(\delta^*_n = \mu_n\) if \(T^*_N = n\).
%     \item[(ii)] The optimal Bayesian risk is \(\rho^*_N = E[R^N_1]\).
% \end{enumerate}

% Therefore, Thm. 2.7.4 suggests that the optimal stopping time is the first time when the Average Posterior Risk \(R^N_n\) associated with the best terminal decision is less or equal to the APR associated with the continuation of observations. In the following, the risk function \(R^N_n\) defined in (2.207) will be referred to as the minimal a posteriori risk (MAPR). Indeed, alternatively, this risk function can be characterized as

% \[
% R^N_n = \underset{T \in \mathcal{M}_{n \leq N}}{\operatorname{ess\,inf}} E[L(\theta_r, \delta^*_T(X^T), X^T) \mid X^n]
% \]

% The backward induction (2.207) reflects Bellman's optimality principle according to which optimization of the multistage process starts from the end (i.e., from the stage \(N\)). At the \(N\)-th stage, we stop w.p. 1 and the MAPR \(R^N\) is equal to the APR \(R^N_n\) associated with the best terminal decision \(\delta^*_n(X^N)\). At the \((N-1)\)-th stage we have two possibilities – either to stop and make an optimal terminal decision, in which case we lose \(R^N_n-1\), or to continue the observations and lose \(R^N_n\). As a result, we stop if \(R^N_{\text{st}} \leq R^N_{n-1}\) and make another observation \(X_N\) otherwise. The MAPR is equal to \(R^N_1 = \min\{R^N_{\text{st}}, R^N_{n-1}\}\). The situation is analogous for any \(n = N, \ldots, 1\), and the minimal average risk \(\rho^*_N = \inf_6 \rho(\delta)\) is equal to \(E[R^N_1]\).




\clearpage

==> DevilsAdvocate_RebuttalSimulation.tex <==
\paragaph{\texttt{FIRMBOUND} is a mere combination of existing works.}


Moreover, major breakthroughs are often based on insightful combination of existing works.
Cite Sugiyama's ICASSP2023 best paper, it's a simple combination but so ingeniously designed to win the award
Also cite SPRT-TANDEM, essentially combination of Bayes rule, DRE, and neural net

\paragraph{It's simple.}
This comment indicates that a problem must be solved with a esoteric method. We respectfully disagree.

\paragaph{Backward induction has already been solved by xxx (e.g., inverse active sensing paper)}
Curse of dimensionality hampers the numerical simulation from operating on real data.

\paragraph{Other ECTS algorithms achieve smaller APRs.}
As we state in Discussion, well-calibrated statistics are necessary to reach the best pareto-front given a sampling cost. No wonder an overconfident model gives smaller APRs.

\paragraph{This is not SOTA.}
Fuck you, I mean, as we stated in Experiments, we aim to have a \textit{fair} comparison across baselines, not to show off the best ``number.''

\paragraph{You still need to search for a good sampling cost. Isn't it the same for searching a good threshold value with SPRT-TANDEM?}
Compute AVR curve on training dataset?

\paragraph{Experimental details are mostly about SPRT-TANDEM, contribution is incremental.}
If one reports Transformer training details on an LLM paper, would you say it's incremental because it's based on Transformer?

\paragraph{Why don't you include classification penalty in APR?} We can, but it's redundant - the consistent estimation of LLRs already handles it. 

\paragraph{The paper is not self-contained. Some proof is missing.} In the era of LLMs, summarize proofs from existing litarature is trivial. Instead of being self-contained, we focus on our contributions to reduce workload of the readers.

\paragraph{Sometimes FIRMBOUND yields higher APR compared with static threshold SPRT. Why?}
Minimizing APR or Bayes risk?

\paragraph{Related work is missing!}
It's in Appendix and hey, the main text already contains >100 papers...


% TM Memo
% イントロ：十分インパクトのある流れになっているか？逆にoverstateしていないか？contributionsのまとめは適切か？（そもそも必要か？）
% Preliminary：CFLに関して、内容は私が書いたものなので(GPTは体裁だけ）慎重に内容を吟味してください。
% Exp & results：実験がちゃんと想像できますか？私は慣れてしまっているので、必要情報が欠けている可能性があります。
% 全体として：ご存知の通り9ページmax、に対し現在11ページありますが、削る（Appendixにまわす）ならどこですか？Referenceは適切に引かれていますか、不足しているものはありますか？

% その他コメント：
% ・permissionなしで自由に編集していただいて構いません。
% ・思いついたreferenceは片っ端から追加してください。ご存知のようにreferenceはページ数にカウントされません。
% ・Appendixにあるoptimalityのまとめ、いまんとこICML版のAppendixをそのまま貼ってるけど…流石に怒られるかねえ。盗作とかなんとか言われて。正直本質的じゃないけど、どうしましょうか。GPTに内容そのままでrephraseさせるのがいいかな？
% ・Conclusionは切ります

==> Statistics.tex <==
\section{Statistics}


==> Supplementary_ICNN.tex <==
\section{On the choice of CFL algorithm.}\label{app:ICNN}

\paragraph{Convergence guarantee on the two-block ADMM algorithm.}
We used the two-block ADMM algorithm in \texttt{FIRMBOUND} for its consistent convex function estimation and faster convergence rate, $ \mathcal{O}\left(\frac{n^3 d^{1.5}}{\epsilon} + \frac{n^2 d^{2.5}}{\epsilon} + \frac{n d^3}{\epsilon}\right) $, where $n, d, \epsilon$ are the number of data points, dimensionality of the data, and desired error~\citeApp{Siahkamari2022CFL}, which is considerably more efficient than the traditional ADMM's $ \mathcal{O}\left(\frac{n^5 d^2}{\epsilon}\right) $.

\paragraph{Input-Convex Neural Networks as an estimator of the conditional probability.} 
As an additional method to estimate the conditional expectation, we experimented with Input-Convex Neural Networks (ICNN~\citeApp{Amos2017ICNN}). ICNNs, which employ non-negative weights and non-decreasing activation functions such as softplus, ensure that the learned function remains convex with respect to its inputs. This characteristic is advantageous in optimization problems, where convexity can facilitate more efficient and robust solutions. However, we observed that ICNNs are overly sensitive to data noise and have difficulty fitting even a simple parabola (Figure \ref{fig:ICNN}), making them unsuitable for real-world applications.


\begin{figure*}[htbp]
    \centerline{\includegraphics[width=14cm,keepaspectratio]{ICNN_parabolafit.pdf}}
    \caption{ICNNs have difficulty fitting even a simple parabola.
        ICNNs are trained on a one-dimensional parabola. 
        The plot shows the perturbed one-dimensional parabola (blue) and its ICNN approximation (orange) after training for 50,000 iterations on 10,000 samples.
        The ground-truth parabola is defined as $y=x^2$ with $x + 0.01 \times \epsilon$, where $x \in [-1, 1]$, and $\epsilon$ is drawn from the standard Gaussian distribution)
        The learning rate decays by a factor of 0.5 every 20,000 iterations. 
        The ICNN has 3 or 5 linear layers with 256 or 1024 hidden units and a softplus activation for each and uses the Adam optimizer with the initial learning rate of 0.01, batch size of 16 or 1024, and no weight decay. The loss function is the mean squared error (MSE) loss.}
        \label{fig:ICNN}
\end{figure*}

\clearpage

==> Supplementary_domain_gap.tex <==
\section{Domain Gap in UCF101 Prevents \texttt{FIRMBOUND} from Reaching the Global Minima}\label{app:domain_gap}
We would like to address the critical concern regarding FIRMBOUND's failure to achieve the global minima of the average a posteriori risk (AAPR) under the UCF101 dataset.

We have identified that the primary reason behind the failure to achieve the global minima on the UCF101 test dataset is the \textbf{domain gap} between the training and test datasets. 

\begin{figure*}[htbp]
\centerline{\includegraphics[width=7cm,keepaspectratio]{UCF101_trainset.pdf}}
\caption{\textbf{Results on the training dataset of UCF101.} }
\end{figure*}
In our additional experiments, we observed that FIRMBOUND does achieve the global minima of AAPR on the UCF101 training dataset. This indicates that our method is capable of optimal performance when the training and test data distributions are aligned. However, the discrepancy between the training and test datasets in UCF101, which reflects a domain gap, has affected the generalizability of our results. 

Fig.~\ref{fig:UCF_domain_gap} illustrates the estimated LLR trajectories for two example classes from the UCF101 dataset. The red and blue trajectories represent the likelihood ratios for two different classes. The LLR trajectories for the training data (left panel) exhibit good separability between the two classes, with clear and distinct increases and decreases in LLR values. In contrast, the LLR trajectories for the test data (right panel) show significantly smaller angles and reduced class separation. The LLRs for the test data have smaller magnitudes and exhibit a delayed increase compared to the training data. This discrepancy indicates a domain gap between the training and test datasets. The smaller magnitude and delayed increase of LLRs in the test data lead to decision delays when applying decision boundaries learned from the training dataset. This phenomenon contributes to the observed failure in achieving the global minima of the average a posteriori risk (AAPR) on the UCF101 test dataset. 

In comparison, the SiW dataset exhibited minimal domain gap between its training and test datasets, as evidenced by consistent LLR trajectories (Fig.~\ref{fig:SiW_domain_gap}). This supports the interpretation that the delayed decision-making observed in the UCF101 dataset, and the successful minimization of AAPR on the SiW dataset, is attributable to the domain gap present in UCF101.

\begin{figure*}[htbp]
\centerline{\includegraphics[width=14cm,keepaspectratio]{UCF1vs2_train_and_test_domaingap.pdf}}
\caption{\textbf{Estimated LLRs on the train and test datasets of UCF101.} }
\label{fig:UCF_domain_gap}
\end{figure*}

\begin{figure*}[htbp]
\centerline{\includegraphics[width=14cm,keepaspectratio]{SiW_train_test_LLRs.pdf}}
\caption{\textbf{Estimated LLRs on the train and test datasets of SiW.} }
\label{fig:SiW_domain_gap}
\end{figure*}

We recognize the importance of addressing domain gaps in machine learning research. However, it is important to note that handling domain gaps is beyond the current scope of our paper, which focuses on developing an optimal stopping rule for early classification within finite horizons. Addressing domain adaptation and transfer learning would require a different methodological approach and additional research efforts. Potential directions include incorporating domain adaptation techniques and robustifying FIRMBOUND against such discrepancies.

\clearpage

==> _Discussion.tex <==
\section{Supplementary discussion}\label{app:discussion}
\paragraph{Why is the SPRT-TANDEM superior to other baselines?}
The potential drawbacks common to the LSTM-s/m and EARLIEST is that they incorporate long temporal correlation: it may lead to (1) the class signature length problem and (2) vanishing gradient problem, as we described in Section 3. (1) If a class signature is significantly shorter than the correlation length in consideration, uninformative data samples are included in calculating the log-likelihood ratio, resulting in a late or wrong decision. (2) long correlations require calculating a long-range of backpropagation, prone to the vanishing gradient problem. 

An LSTM-s/m-specific drawback is similar to that of Neyman-Pearson test, in the sense that it fixes the number of samples before performance evaluations. On the other hand, the SPRT, and the SPRT-TANDEM, classify various lengths of samples: thus, the SPRT-TANDEM can achieve a smaller sampling number with high accuracy on average. Another potential drawback of LSTM-s/m is that their loss function explicitly imposes monotonicity to the scores. While the monotonicity is advantageous for quick decisions, it may sacrifice flexibility: the LSTM-s/m can hardly change its mind during a classification.

EARLIEST, the reinforcement-learning based classifier, decides on the various length of samples. A potential EARLIEST-specific drawback is that deep reinforcement learning is known to be unstable (\citeApp{Nikishin2018, Kumar2020}).

\paragraph{How optimal is the SPRT-TANDEM?} In practice, it is difficult to strictly satisfy the necessary conditions for the SPRT's optimality (Theorem \ref{thm:iid optimality} and \ref{thm:non-iid optimality}) because of experimental limitations. 

One of our primary interests is to apply the SPRT, the provably optimal algorithm, to real-world datasets. A major concern about extending Wald's SPRT is that we need to know the true likelihood ratio a priori to implement the SPRT. Thus we propose the SPRT-TANDEM with the help of machine learning and density ratio estimation to remove the concern, if not completely. However, some technical limitations still exist. Let us introduce two properties of the SPRT that can prevent the SPRT-TANDEM from approaching exact optimality.

Firstly, the SPRT is assumed to terminate for all the LLR trajectories under consideration with probability one. The corresponding equation stating this assumption is Equation (\ref{eq:i.i.d. termination}) and (\ref{eq:non-i.i.d. termination}) under the i.i.d. and non-i.i.d. condition, respectively. Given that this assumption (and the other minor technical conditions in Theorem \ref{thm:iid optimality} and \ref{thm:non-iid optimality}) is satisfied, \textit{the more precisely we estimate the LLRs, the more we approach the genuine SPRT implementation and thus its asymptotic Bayes optimality.} 

Secondly, the non-i.i.d. SPRT is asymptotically optimal when the maximum number of samples allowed is not fixed (\textit{infinite horizon}). On the other hand, our experiment truncates the SPRT (\textit{finite horizon}) at the maximum timestamp, which depends on the datasets. Under the truncation, gradually collapsing thresholds are proven to give the optimal stopping (\citeApp{TartarBook}); however, the collapsing thresholds are obtained via backward induction (\citeApp{Bingham2006}), which is possible only after observing the \textit{full} sequence. Thus, under the truncation, finding the optimal solutions in a strict sense critically limits practical applicability.  

The truncation is just an experimental requirement and is not an essential assumption for the SPRT-TANDEM. Under the infinite horizon settings, the LLRs is assumed to increase or decrease toward the thresholds (Theorem \ref{thm:non-iid optimality}) in order to ensure the asymptotic optimality. However, we observed that the estimated LLRs tend to be asymptotically flat, especially when $N$ is large (Figure \ref{fig:NMNIST_LLR}, \ref{fig:UCF_LLR}, and \ref{fig:SiW_LLR}); the estimated LLRs can violate the assumption of Theorem \ref{thm:non-iid optimality}.
%Therefore, neither the truncated SPRT-TANDEM with non-collapsing thresholds nor non-truncated SPRT-TANDEM is not strictly optimal.

One potential reason for the flat LLRs is the TANDEM formula: the first and second term of the formula has a different sign. Thus, the resulting log-likelihood ratio will be updated only when the difference between the two terms are non-zero. Because the first and second term depends on $N+1$ and $N$ inputs, respectively, it is expected that the contribution of one input becomes relatively small as $N$ is enlarged. We are aware of this issue and already started working on it as future work.  

Nevertheless, the flat LLRs at least do not spoil the practical efficiency of the SPRT-TANDEM, as our experiment shows. In fact, because we cannot know the true LLR of real-world datasets, it is not easy to discuss whether the assumption of the increasing LLRs is valid on the three databases (NMNIST, UCF, and SiW) we tested. Numerical simulation may be possible, but it is out of our scope because our primary interest is to implement a practically usable SPRT under real-world scenarios. 

% The sequential probability ratio test is a powerful test reaches a user-defined mean classification accuracy with a much smaller sample size than its fixed-sample test counterpart, the Neyman-Pearson test. However, SPRT has rarely been considered practical for modern time-series classification tasks because it has two strict assumptions. First, SPRT assumes i.i.d. samples. This indicates that the random shuffling of the samples does not affect the classification results, which is overly optimistic in the case of time-series data that may have higher-order correlations. Second, although the original SPRT gets the most advantage from the given likelihoods, it does not consider \textit{how} to estimate the likelihoods during the sequential samplings. We have overcome these difficulties by devising a novel algorithm to calculate LLRs by allowing up to Nth-order correlations between samples, a much more relaxed assumption than i.i.d. The likelihood ratio is estimated from the outputs of a neural network consisting of two compartments, the feature extractor, and the temporal integrator. Aided by the LLLR, our network implementing the N-SPRT algorithm outperforms fixed-sample counterarts, such as convolutional LSTM or 3DResNet, despite it having a smaller sample size. 

% A significant practical advantage of SPRT is that the user can set the desired classification accuracy by tuning the hyperparameters $\alpha$ and $\beta$. By taking a linear programming approach, Wald showed that the actual error rates, FAR and FRR, are bounded in a quadrangle (Fig. \ref{fig:WaldLinear}, \citep{WaldBook}). As expected from this theoretical consideration, the 3D-ness detection experiment showed small FAR and FRR values inside the quadrangle. However, Wald's linear programming conjecture assumes that the data series is i.i.d. In the future, we will perform a theoretical analysis assessing the effect of LLR estimation error on the quadrangle.
% % \begin{figure}[htbp]
% % \centerline{\includegraphics[width=8cm,keepaspectratio]{../WaldLinear.pdf}}
% % \caption{Wald's linear programming showing possible values of $\alpha$ and $\beta$ in red, given the threshold A and B.}
% % \label{fig:WaldLinear} 
% % \end{figure}
% Unlike fixed-sample classifiers such as convolutional LSTM or ResNet, N-SPRT can take variable length input sequences and make a fast decision on samples that are easy to classify, while at the same time allowing for longer times to make careful decisions on difficult samples. SPRT is thus in line with a human's way of making decisions. In a fastest-finger-first quiz, for example, a respondent waits and listens to the question until he or she collects a sufficient amount of information to give a correct answer. Corroborating this intuitive decision strategy, the neurons in the LIP area show activities proportional to the LLR \citeApp{Kirasan}. N-SPRT makes the most of this neural algorithm to minimize the classification error and the expected sample size as much as possible.

\paragraph{The best order $N$ of the SPRT-TANDEM.}
The order $N$ is a hyperparamer, as we mentioned in Section \ref{sec:SPRT-TANDEM} and thus needs to be tuned to attain the best performance. However, each dataset has its own temporal structure, and thus it is challenging to acquire the best order a priori. In the following, we provide a rough estimation of the best order, which may give dramatic benefit to the users and may lead to exciting future works.

Let us introduce a concept, \textit{specific time scale}, which is used in physics to analyze qualitative behavior of a physical system. 
Here, we define the specific time scale of a physical system as a temporal interval in which the physical system develops dramatically. For example, suppose that a physical system under consideration is a small segment of spacetime in which an unstable particle, ortho-positronium (o-Ps), exists. In this case, a specific time scale can be defined as the lifetime of o-Ps, $0.14 \mu s$ (\citeApp{czarnecki1999positronium}), because the o-Ps is likely to vanish in $0.14 \times O(1) \mu s$ --- the physical system has changed completely. Note that the definition of specific time scale is not unique for one physical system; it depends on the phenomena the researcher focuses on. Specific (time) scale are often found in fundamental equations that describes physical systems. In the example above, the decay equation $N(t) = A \exp (- t / \ta)$ has the lifetime $\ta \in \mbr$ in itself. Here $N(t) \in \mbr$ is the expected number of o-Ps' at time $t \in \mbr$, and $A \in \mbr$ is a constant.

Let us borrow the concept of the specific time scale to estimate the best order of the SPRT-TANDEM before training neural networks, though there is a gap in scale. In this case, we define the specific time scale of a dataset as the number of frames after which a typical video in the dataset shows completely different scene. As is discussed below, we claim that \textit{the specific time scale of a dataset is a good estimation of the best order of the SPRT-TANDEM}, because the correlations shorter than the specific time scale are insufficient to distinguish each class, while the longer correlations may be contaminated with noise and keep redundant information.

First, we consider Nosaic MNSIT (NMNIST). The specific time scale of NMNIST can be defined as the half-life\footnote{
This choice of words is, strictly speaking, not correct, because the noise decay in NMNIST is \textit{linear}; the definition of half-life in physics assumes the decay to be \textit{exponential}.
} of the noise, i.e., the necessary temporal interval for half of the noise to disappear. It is 10 frames by definition of NMNIST, and approximately matches the best order of the SPRT-TANDEM: in Figure \ref{fig:ExpResult}, our experiment shows that the 10th order SPRT-TANDEM (with 11-frames correlation) outperforms the other orders in the latter timestamps, though we did not perform experiments with all the possible orders. A potential underlying mechanism is: Too long correlations keep noisy information in earlier timestamps, causing degradation, while too short correlations do not fully utilize the past information.

Next, we discuss the two classes in UCF101 action recognition database, handstand pushups and handstand walking, which are used in our experiment. A specific time scale is $\sim 10$ frames because of the following reasons. The first class, handstand pushups, has a specific time scale of one cycle of raising and lowering one's body $\sim 50$ frames (according to the shortest video in the class). The second class, handstand walking, has a specific time scale of one cycle of walking, i.e., two steps, $\sim 10$ frames (according to the longest video in the class). Therefore the specific time scale of UCF is $\sim 10$, the smaller one, since we can see whether there is a class signature in a video within at most $\sim 10$ frames. The specific time scale matches the best order of the SPRT-TANDEM according to Figure \ref{fig:ExpResult}.

Finally, a specific time scale of SiW is $\sim 1$ frame, because a single image suffices to distinguish a real person and a spoofing image, because of the reflection of the display, texture of the photo, or the movement specific to a live person\footnote{
In fact, the feature extractor, which classified a single frame to two classes, showed fairly high accuracy in our experiment, without temporal information.
}. The best order in Figure \ref{fig:ExpResult} is $\sim 1$, matching the specific time scale.

We make comments on two potential future works related to estimation of the best order of the SPRT-TANDEM. First, as our experiments include only short videos, it is an interesting future work to estimate the best order of the SPRT-TANDEM in super-long video classification, where gradient vanishing becomes a problem and likelihood estimation becomes more challenging. Second, it is an exciting future work to analyse the relation of the specific time scale to the best order when there are multiple time scales. For example, recall the discussion of locality above in this Appendix \ref{app:discussion}: Applying the SPRT-TANDEM to a dataset with distributed class signatures is challenging. Distributed class signatures may have two specific time scales: e.g., one is the mean length of the signatures, and the other is the mean interval between the signatures.

% AFE on Nov.15th: commented out for being overlapped with the optimality discussion
% \paragraph{Forced decision making at the last frame: truncated SPRT.}
% The original SPRT continues observations until LLR reaches either of the two thresholds; however, since sequence sizes are finite in real experiments, we collapse the thresholds to be 0 at the last frame to finish all the decisions, as mentioned in Section \ref{experiments}. This variant of the SPRT is called the truncated SPRT (\citeApp{TartarBook}). Therefore, strictly speaking, the algorithm employed in our experiment is the truncated SPRT. 

% However, the optimality of the truncated SPRT was proven as well (\citeApp{TartarBook}), given ``appropriately'' collapsing, time-dependent thresholds. Thus it may be an interesting future work to implement the truncated SPRT with the optimal collapsing thresholds, but computing the optimal thresholds is a big challenge, because of its extremely high computational cost.
\paragraph{The best threshold $\lambda_{\tau^*}$ of the SPRT-TANDEM.}
In practice, a user can change the thresholds after deploying the SPRT-TANDEM algorithm once and control the speed-accuracy tradeoff. Computing the speed-accuracy-tradeoff curve is not expensive, and importantly computable without re-training. According to the speed-accuracy-tradeoff curve, a user can choose the desired accuracy and speed. Note that this flexible property is missing in most other deep neural networks: controlling speed usually means changing the network structures and training it all over again.

\paragraph{End-to-end v.s. separate training.} 
The design of SPRT-TANDEM does not hamper an end-to-end training of neural networks; the feature extractor and temporal integrator can be readily connected for thorough backpropagation calculation. However, in Section \ref{experiments}, we trained the feature integrator and temporal integrator separately: after training the feature integrator, its trainable parameters are fixed to start training the temporal integrator. We decided to train the two networks separately because we found that it achieves better balanced accuracy and mean hitting time. Originally we trained the network using NMNIST database with an end-to-end manner, but the accuracy was far lower than the result reported in Section \ref{experiments}. We observed the same phenomenon when we trained the SPRT-TANDEM on our private video database containing 1-channel infrared videos. These observations might indicate that while the separate training may lose necessary information for classification compared to the end-to-end approach, it helps the training of the temporal integrator by fixing information at each data point. It will be interesting to study if this is a common problem in early-classification algorithms and find the right balance between the end-to-end and separate training to benefit both approaches.


\paragraph{Feedback to the field of neuroscience.}\citeApp{Kirasan} experimentally showed that the SPRT could explain neural activities in the area LIP at the macaque parietal lobe. They randomly presented a sequence of visual objects with associated reward probability. A natural question arises from here: what if the presented sequence is not random, but a time-dependent visual sequence? Will the neural activity be explained by our SPRT-TANDEM, or will the neurons utilize a completely different algorithm? Our research provides one driving hypothesis to lead the neuroscience community to a deeper understanding of the brain's decision-making system.

\paragraph{Usage of statistical tests.}As of writing this manuscript, not all of the computer science papers use statistical tests to evaluate their experiments. However, in order to provide an objective comparison across proposed and existing models, running multiple validation trials with random seeds followed by a statistical test is helpful. Thus, the authors hope that our paper stimulates the field of computer science to utilize statistical tests more actively.

\paragraph{Ethical concern.}The proposed method, SPRT-TANDEM, is a general algorithm applicable to a broad range of serial data, such as auditory signals or video frames. Thus, any ethical concerns entirely depend on the application and training database, not on our algorithm \textit{per se}. For example, if SPRT-TANDEM is applied to a face spoofing detection, using faces of people of one particular racial or ethnic group as training data may lead to a bias toward or against people of other groups. However, this bias is a concern in machine learning in general, not specific to the SPRT-TANDEM.

\paragraph{Is the SPRT-TANDEM ``too local''?}
In our experiments in Section \ref{experiments}, the SPRT-TANDEM with maximum correlation allowed (i.e., 19th, 49th, and 49th on NMNIST, UCF, and SiW databases, respectively) does not necessarily reach the highest accuracy with a larger number of frames. Instead, depending on the database, the lower order of approximation, such as 10th order TANDEM, outperforms the other orders. In the SiW database, this observation is especially prominent: the model records the highest balanced accuracy is the 2nd order SPRT-TANDEM. While this may indicate our TANDEM formula with the ``dropping correlation'' strategy works well as we expected, a remaining concern is the SPRT may integrate too local information. What if class signatures are far separated in time? 

In such a case, the SPRT-TANDEM may fail to integrate the distributed class signatures for correct classification. On the other hand, the SPRT-TANDEM may be able to add the useful information of the class signatures to the LLR only when encountering the signatures (in other words, do not add non-zero values to the LLR without seeing class signatures). The SPRT-TANDEM may be able to skip unnecessary data points without modification, or with a modification similar to  SkipRNN (\citeApp{SkipRNN}), which actively achieve this goal: by learning unnecessary data point, the SkipRNN skips updating the internal state of RNN to attend just to informative data. Similarly, we can modify the SPRT-TANDEM so that it learns to skip updating LLR upon encountering uninformative data. It will be exciting future work, and the authors are looking forward to testing the SPRT-TANDEM on a challenging database with distributed class signatures.

\paragraph{A more challenging dataset: Nosaic MNIST-Hard (NMNIST-H).}
In the main text, we see the accuracy of the SPRT-TANDEM saturates within a few timestamps. Therefore, it is worth testing the models on a dataset that require more samples for reaching good performance. We create a more challenging dataset, \textit{Nosaic MNIST-Hard}: The MNIST handwritten digits are buried with heavier noise than the orifinal NMNIST (only 10 pixels/frame are revealed, while it is 40 pixels/frame for the original NMNIST). The resulting speed-accuracy tradeoff curves below show that the SPRT-TANDEM outperforms LSTM-s/m more than the error-bar range, even on the more challenging dataset requiring more timestamps to attain the accuracy saturation.

\begin{figure}[htbp]
    \centerline{\includegraphics[width=15cm,keepaspectratio]{./img/binNMNIST-H.pdf}}
    \caption{The speed-accuracy tradeoff curve. Compare this with Figure \ref{fig:ExpResult} in the main text. "10th TANDEM" means the 10-th order SPRT-TANDEM. "19th TANDEM" means the 19-th order SPRT-TANDEM.
    The numbers of trials for hyperparameter tuning if 200 for all the models. The error bars are standard error of mean (SEM). The numbers of trials for statistics are 440, 240, 200, and 200 for 10th TANDEM, 19th TANDEM, LSTM-s, and LSTM-m, respectively.}
\end{figure}
\newpage

==> _Optimality.tex <==
% TM Defined Aliases 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\nn{\nonumber \\ }
\def\no{\nonumber }
\def\ti{\tilde}
\def\mc{\mathcal} % hypothesis class \mc{H}, true distribution\mc{D} etc.
\def\mb{\mathbb} %\mb{N}: natural number
\def\mbm{\mathbbm} %\mbm{1}: indicator fcn
\def\mr{\mathrm} % sup, exp, ...
\def\mf{\mathfrak} % German math symbols. Rademacher complexity\mf{R} etc.
\def\f{\frac}
\def\lt{\left}
\def\r{\right}
\def\rt{\right}
\def\sr{\sqrt}
\def\pl{\partial}
% Math new commands
% \newcommand{\argmax}{\mathop{\rm argmax}\limits}
% \newcommand{\argmin}{\mathop{\rm argmin}\limits}
% Other aliases
\def\n{\newline } % equivalent to \\
\def\protl{\protect \linebreak } %used when linebreaking in caption
\def\bs{\backslash} % $\backslash$
\def\ttt{\texttt} % \texttt{blah} is {\tt blah}
\def\fns{\footnotesize} % 8pt; default=10pt {\fns ...}
\def\ttf{\tt \footnotesize }
\def\mbr{\mathbb{R}} 
\def\mbq{\mathbb{Q}}
\def\mbz{\mathbb{Z}}
\def\mbn{\mathbb{N}}
\def\mbp{\mathbb{P}}
\def\mbe{\mathbb{E}}
\def\mcd{\mathcal{D}}
\def\mcx{\mathcal{X}}
\def\mcy{\mathcal{Y}}
\def\mcz{\mathcal{Z}}
\def\mch{\mathcal{H}}
\def\mcf{\mathcal{F}}
\def\mca{\mathcal{A}}
\def\mcn{\mathcal{N}}
\def\mco{\mathcal{O}}
\def\mcp{\mathcal{P}}
\def\mce{\mathcal{E}}
\def\mfr{\mathfrac{R}}
% Aliases of Greek characters
\def\al{\alpha}
\def\be{\beta}
\def\ga{\gamma}
\def\de{\delta}
\def\ep{\epsilon}
\def\ze{\zeta}
\def\et{\eta}
\def\th{\theta}
\def\io{\iota}
\def\ka{\kappa}
\def\la{\lambda}
\def\rh{\rho}
\def\si{\sigma}
\def\ta{\tau}
\def\up{\upsilon}
\def\ph{\phi}
\def\ch{\chi}
\def\ps{\psi}
\def\om{\omega}
\def\Al{A}
\def\Be{B}
\def\Ga{\Gamma}
\def\De{\Delta}
\def\Ep{E}
\def\Ze{Z}
\def\Et{H}
\def\Th{\Theta}
\def\Io{I}
\def\Ka{K}
\def\La{\Lambda}
\def\Rh{P}
\def\Si{\Sigma}
\def\Ta{T}
\def\Up{\Upsilon}
\def\Ph{\Phi}
\def\Ch{X}
\def\Ps{\Psi}
\def\Om{\Omega}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Theoretical Aspects of the Sequential Probability Ratio Test} \label{app:optimality_detailed}
In this section, we review the mathematical background of SPRT following the discussion in \citeApp{TartarBook}. First, we define SPRT based on the measure theory and introduce Stein's lemma, which assures the termination of SPRT. To define the optimality of SPRT, we introduce two performance metrics that measure the false alarm rate and the expected stopping time, and discuss their tradeoff --- SPRT solves it. Through this analysis, we utilize two important approximations, the asymptotic approximation, and the no-overshoot approximation, which play essential roles to simplify our analysis. The asymptotic approximation assumes the upper and lower thresholds are infinitely far away from the origin, being equivalent to making the most careful decision to reduce the error rate, at the expense of the stopping time. On the other hand, the no-overshoot approximation assumes that we can neglect the threshold overshoots of the likelihood ratio.

    Next, we show the superiority of SPRT to the Neyman-Pearson test, using a simple Gaussian model. The Neyman-Pearson test is known to be optimal in the two-hypothesis testing problem and is often compared with SPRT. Finally, we introduce several types of optimal conditions of SPRT.     
    \subsection{Preliminaries}\label{sec:preliminaries}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \paragraph{Notations.}Let $(\Om, \mcf, P)$ be a probability space; $\Om$ is a sample space, $\mcf\subset\mcp^{\Om}$ is a sigma-algebra of $\Om$, where $\mcp^A$ denotes the power set of a set $A$, and $P$ is a probability measure. Intuitively, $\Om$ represents the set of all the elementary events under consideration, e.g., $\Om = \{$all the possible elementary events such that "a human is walking through a gate."$\}$. $\mcf$ is defined as a set of the subsets of $\Om$, and stands for all the possible combinations of the elementary events; 
        e.g., $\mcf \ni \{$ "Alice is walking through the gate at the speed of 80 m/min," "Bob is walking through the gate at the speed of 77 m/min," or "Nothing happened."$\}$ $P: \mcf \rightarrow [0, 1]$ is a probability measure, a function that is normalized and countably additive; i.e., $P$ measures the probability that the event $A\in\mcf$ occurs. A random variable $X$ is defined as the measurable function from $\Om$ to a measurable space, practically $\mbr^{d}$ ($d\in\mbn$); e.g., if $\om(\in\Om)$ is "Bob is walking through the gate with a big smile," then $X(\om)$ may be 100 frames of the color images with 128$\times$128 pixels ($d=128\times 128\times 3\times 100$), i.e., a video recorded with a camera attached at the top of the gate. The probability that a random variable $X$ takes a set of values $S\in\mbr^{d}$ is defined as $P(X\in S) := P(X^{-1}(S))$, where $X^{-1}$ is the preimage of $X$. By definition of the measurable function, $X^{-1}(S)\in\mcf$ for all $S \in \mbr^d$. Let $\{ \mcf_t \}_{t\geq0}$ be a filtration. By definition, $\{ \mcf_t \}_{t\geq0}$ is a non-decreasing sequence of sub-sigma-algebras of $\mcf$; i.e., $\mcf_s \subset \mcf_t \subset \mcf$ for all $s$ and $t$ such that $0<s<t$. Each element of filtration can be interpreted as the available information at a given point $t$. $(\Om, \mcf, \{ \mcf_t \}_{t\geq0}, P)$ is called a filtered probability space. 
        
As in the main manuscript, let $X^{(1,T)} := \{ x^{(t)} \}_{t=1}^{T}$ be a sequential data point sampled from the density $p$, where $T\in\mbn\cup\{\infty\}$. For each $t\in[T]$, $x^{(t)}\in\mbr^{d_x}$, where $d_x\in\mbn$ is the dimensionality of the input data. In the i.i.d. case, $p(X^{(1,T)}) = \prod_{t=1}^{T}f(x^{(t)})$, where $f$ is the density of $x^{(1)}$. For each time-series data $X^{(1,T)}$, the associated label $y$ takes the value 1 or 0; we focus on the binary classification, or equivalently the two-hypothesis testing throughout this paper. When $y$ is a class label, $p(X^{(1,T)}|\th)$ is the likelihood density function. Note that $X^{(1,T)}$ with label $y$ is sampled according to density $p(X^{(1,T)}|y)$.
            
Our goal is, given a sequence $X^{(1,T)}$, to identify which one of the two densities $p_1$ or $p_0$ the sequence $X^{(1,T)}$ is sampled from; formally, to test two hypotheses $H_1: y=1$ and $H_0: y=0$ given $X^{(1,T)}$. The decision function or test of a stochastic process $X^{(1,T)}$ is denoted by $d(X^{(1,T)}): \Om \rightarrow \{1,0\}$. We can identify this definition with, for each realization of $X^{(1,T)}$, $d: \mbr^{d_x\times T} \rightarrow \{1,0 \}$, i.e., $X^{(1,T)} \mapsto y$, where $y\in\{1,0\}$. Thus we write $d$ instead of $d(X^{(1,T)})$, for simplicity. The stopping time of $X^{(1,T)}$ with respect to a filtration $\{ \mcf_t \}_{t\geq0}$ is defined as $\ta:=\ta(X^{(1,T)}): \Om\rightarrow\mbr_{\geq0}$ such that $\{\om\in\Om|\ta(\om)\leq t \}\in\mcf_t$. Accordingly, for fixed $T\in\mbn\cup\{\infty\}$ and $y \in \{1,0\}$, $\{d=y \}$ means the set of time-series data such that the decision function accepts the hypothesis $H_i$ with a finite stopping time; more specifically, $\{d=y \} = \{\om\in\Om| d(X^{(1,T)})(\om) = y, \ta(X^{(1,T)})(\om)<\infty\}$. The decision rule $\de$ is defined as the doublet $(d,\ta)$. Let $\La_T := \La(X^{(1,T)}) := \f{p(X^{(1,T)}|y=1)}{p(X^{(1,T)}|y=0)}$ and $\la_T := \log \La_T$ be the likelihood ratio and the log-likelihood ratio of $X^{(1,T)}$. In the i.i.d. case, $\La_T = \prod_{t=1}^T \f{p(x^{(t)}|y=1)}{p(x^{(t)}|y=0)} = \prod_{t=1}^T Z^{(t)}$, where $p(X^{(1,T)}|y) = \prod_{t=1}^T p(x^{(t)}|y)\,$ ($y\in\{1,0\}$) and $Z^{(t)} := \f{p(x^{(t)}|y=1)}{p(x^{(t)}|y=0)}$.

    

    \subsection{Definition and the Tradeoff of False Alarms and Stopping Time}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        Let us overview the theoretical structure of SPRT. In the following, we assume that the time-series data points are i.i.d. until otherwise stated.
        \paragraph{Definition of SPRT.}The sequential probability ratio test (SPRT), denoted by $\de^*$ is defined as the doublet of the decision function and the stopping time.
            \begin{definition}{\bf Sequential probability ratio test (SPRT)}\mbox{}\\
                Let $a_0 = -\log A_0 \geq 0$ and $a_1 = \log A_1\geq 0$ be (the absolute values of) a lower and an upper threshold respectively.
                \begin{equation}
                    \de^* = (d^*, \ta^*),
                \end{equation}
                \begin{eqnarray}
                    d^*(X^{(1,T)}) =
                    \begin{cases}
                        1 &\textrm{if $\la_{\ta^*}\geq a_1$} \\
                        0 &\textrm{if $\la_{\ta^*}\leq -a_0$} \, ,
                    \end{cases}
                \end{eqnarray}
                \begin{equation}
                    \ta^* = \mr{inf}\{ T\geq 0 | \la_T \notin (-a_0, a_1) \} \, .
                \end{equation}
            \end{definition}
            Note that $d^*$ and $\ta^*$ implicitly depend on a stochastic process $X^{(1,T)}$. In general, a doublet $\de$ of a terminal decision function and a stopping time is called a decision rule or a hypothesis test.
    
        \paragraph{Termination.}The i.i.d.-SPRT terminates with probability one and all the moments of the stopping time are finite, provided that the two hypotheses are distinguishable:
            %* continuous time ?
            \begin{lemma}{\bf Stein's lemma}\mbox{}\\
                Let $(\Om, \mcf, P)$ be a probability space and $\{Y^{(t)}\}_{t\geq 1}$ be a sequence of i.i.d. random variables under $P$. Define $\ta := \mr{inf}\{T\geq1|\sum_{t=1}^T Y^{(t)}\notin(-a_0, a_1)\}$. If $P(Y^{(1)}) \neq 1$, the stopping time $\ta$ is exponentially bounded; i.e., there exist constants $C>0$ and $0<\rh<1$ such that $P(\ta>T) \leq C\rh^T$ for all $T\geq1$. Therefore, $P(\ta<\infty)=1$ and $\mbe[\ta^k]<\infty$ for all $k>0$.
            \end{lemma}

        \paragraph{Two performance metrics.}Considering the two-hypothesis testing, we employ two kinds of performance metrics to evaluate the efficiency of decision rules from complementary points of view: the false alarm rate and the stopping time. The first kind of metrics is the operation characteristic, denoted by $\be(\de,y)$, and its related metrics. The operation characteristic is the probability of the decision being 0 when the true label is $y=y$; formally, 
            \begin{definition}{\bf Operation characteristic}\mbox{}\\
                The operation characteristic is the probability of accepting the hypothesis $H_0$ as a function of $y$: 
                \begin{equation}
                    \be(\de,y) := P(d=0|y) \, .
                \end{equation}
            \end{definition}
            Using the operation characteristic, we can define four statistical measures based on the confusion matrix; namely, False Positive Rate (FPR), False Negative Rate (FNR), True Negative Rate (TNR), and True Positive Rate (TPR).
            \begin{align}
                & \textrm{FPR: }\, \al_0(\de) := 1-\be(\de, 0) = P(d=1|y=0)\\
                & \textrm{FNR: }\, \al_1(\de) := \be(\de, 1) = P(d=0|y=1)\\
                & \textrm{TNR: }\, \be(\de, 0) = 1 - \al_0(\de) = 1 - P(d=1|y=0)\\
                & \textrm{TPR: }\, 1- \be(\de, 1) = 1 - \al_1(\de) = 1 - P(d=0|y=1)
            \end{align}
            Note that balanced accuracy is denoted by $(1 + \be(\de, 0) - \be(\de, 1) )/2$ according to this notation. The second kind of metrics is the mean hitting time, and is defined as the expected stopping time of the decision rule:
            \begin{definition}{\bf Mean hitting time}
                The mean hitting time is the expected number of time-series data points that are necessary for testing a hypothesis when the true parameter value is $y$: $\mbe_y \ta = \int_\Om \ta dP(\cdot|y)$. The mean hitting time is also referred to as the expected sample size of the average sample number.
            \end{definition}

            There is a tradeoff between the false alarm rate and the mean hitting time. For example, the quickness may be sacrificed, if we use a decision rule $\de$ that makes careful decisions, i.e., with the false alarm rate $1-\be(\de, 0)$ less than some small constant. On the other hand, if we use $\de$ that makes quick decisions, then $\de$ may make careless decisions, i.e., raise lots of false alarms because the amount of evidences is insufficient. At the end of this section, we show that SPRT is optimal in the sense of this tradeoff.
            
        \paragraph{The tradeoff of false alarms and stopping times for both i.i.d. and non-i.i.d.}We formulate the tradeoff of the false alarm rate and the stopping time. We can derive the fundamental relation of the threshold to the operation characteristic in both i.i.d. and non-i.i.d. cases (\citeApp{TartarBook}):
            \begin{eqnarray}
                \begin{cases}
                    & \al_1^{*} \leq e^{{-a_0}}(1-\al_0^{*}) \\
                    & \al_0^{*} \leq e^{{-a_1}}(1-\al_1^{*}) \label{eq:exact}\, ,
                \end{cases}
            \end{eqnarray}
            where we defined $\al_y^{*} := \al_y(\de^*)$ ($y\in\{1,0\}$). These inequalities essentially represent the tradeoff of the false alarm rate and the stopping time. For example, as the thresholds $a_y$ ($y\in\{1,0\}$) increase, the false alarm rate and the false rejection rate decrease, as (\ref{eq:exact}) suggests, but the stopping time is likely to be larger, because more observations are needed to accumulate log-likelihood ratios to hit the larger thresholds.
            
        \paragraph{The asymptotic approximation and the no-overshoot approximation.}Equation \ref{eq:exact} is an example of the tradeoff of the false alarm rate and the stopping time; further, we can derive another example in terms of the mean hitting time. Before that, we introduce two types of approximations that simplify our analysis. 
            
        The first one is the no-overshoot approximation. It assumes to ignore the threshold overshoots of the log-likelihood ratio at the decision time. This approximation is valid when the log-likelihood ratio of a single frame is sufficiently small compared to the gap of the thresholds, at least around the decision time. On the other hand, the second one is the asymptotic approximation, which assumes $a_0, a_1 \rightarrow \infty$, being equivalent to sufficiently low false alarm rates and false rejection rates at the expense of the stopping time. These approximations drastically facilitate the theoretical analysis; in fact, the no-overshoot approximation alters (\ref{eq:exact}) as follows (see \citeApp{TartarBook}):
        \begin{equation}
            \al_1^{*} \approx e^{{-a_0}}(1-\al_0^{*}), \hspace{15pt} \al_0^{*} \approx e^{{-a_1}}(1-\al_1^{*}) \, ,
        \end{equation}        
        which is equivalent to        
        \begin{align}
            \hspace{5pt}& \al_0^* \approx \f{
                e^{a_0}-1
            }{
                e^{a_0 + a_1}-1
            }, \hspace{15pt}\al_1^* \approx \f{
                e^{a_1}-1
            }{
                e^{a_0 + a_1}-1
            }
            \\
            \Longleftrightarrow\hspace{5pt}& -a_0 \approx \log\left( \f{\al_1^*}{1-\al_0^*} \right), \hspace{10pt} a_1 \approx \log\left( \f{1-\al_1^*}{\al_0^*} \right)\\
            \Longleftrightarrow\hspace{5pt}& \be^*(0) \approx \f{e^{a_1} - 1}{e^{a_1} - e^{-a_0}},\hspace{10pt} \be^*(1) \approx \f{e^{-a_1}-1}{e^{-a_1} - e^{a_0}} \, ,
        \end{align}
        where $\be^*(y) := \be(\de^*, y)$ ($y\in\{1,0\}$). Further assuming the asymptotic approximation, we obtain 
        \begin{equation}
            \al_0^* \approx e^{-a_1}, \quad \al_1^* \approx e^{-a_0}.\label{eq:asymptotic}
        \end{equation}
        Therefore, as the threshold gap increases, the false alarm rate and the false rejection rate decrease exponentially, while the decision making becomes slow, as is shown in the following.            
        
        \paragraph{Mean hitting time without overshoots.}Let $I_y := \mbe_y[Z^{(1)}]$ ($y\in\{1,0\}$) be the Kullback-Leibler divergence of $f_1$ and $f_0$. $I_y$ is larger if the two densities are more distinguishable. Note that $I_y \gneq 0$ since $P_y (Z^{(1)}=0) \lneq 1$, and thus the mean hitting times of SPRT without overshoots are expressed as 
            \begin{align}
                \mbe_1[\ta^*] &= \f{1}{I_1} \left[(1-\al_1^*) \log(\f{1-\al_1^*}{\al_0^*}) - \al_1^* \log(\f{1-\al_0^*}{\al_1^*} )  \right]  \, ,\label{eq:mean_hitting_time_no_overshoot1}\\
                \mbe_0[\ta^*] &= \f{1}{I_0} \left[(1-\al_0^*) \log(\f{1-\al_0^*}{\al_1^*}) - \al_0^* \log(\f{1-\al_1^*}{\al_0^*} )  \right] \, \label{eq:mean_hitting_time_no_overshoot0}
            \end{align}
            In \citeApp{TartarBook}. Introducing the function
            \begin{equation}
                \ga(x,y) := (1-x) \log(\f{1-x}{y}) - x \log(\f{1-y}{x}) \, ,
            \end{equation}
            we can simplify (\ref{eq:mean_hitting_time_no_overshoot1}-\ref{eq:mean_hitting_time_no_overshoot0}):
            \begin{align}
                \mbe_1[\ta^*] &= \f{1}{I_1} \ga(\al_1^*, \al_0^*) \label{eq:tau = alpha1} \\
                \mbe_0[\ta^*] &= \f{1}{I_1} \ga(\al_0^*, \al_1^*) \, . \label{eq:tau = alpha2}
            \end{align}
            (\ref{eq:mean_hitting_time_no_overshoot1}-\ref{eq:mean_hitting_time_no_overshoot0}) shows the tradeoff as we mentioned above: the mean hitting time of positive (negative) data diverges if we are to set the false alarm (rejection) rate to be zero.
        
        \paragraph{The tradeoff with overshoots.}Introducing the overshoots explicitly, we can obtain the equality, instead of the inequality such as (\ref{eq:exact}), that connects the the error rates and the thresholds. We first define the overshoots of the thresholds $a_0$ and $a_1$ at the stopping time as 
            \begin{align}
                & \ka_1(a_0,a_1) := \la_{\ta^*} - a_1    &&\textrm{on} \{\la_{\ta*}\geq a_1 \} \, \\
                & \ka_0(a_0,a_1) := -(\la_{\ta^*} + a_0) &&\textrm{on} \{\la_{\ta^*} \leq -a_0 \}. 
            \end{align}
            We further define the expectation of the exponentiated overshoots as 
            \begin{align}
                &  e_1(a_0,a_1) := \mbe_1[e^{-\ka_1(a_0,a_1)} | \la_{\ta^*} \geq a_1 ]\, \\
                &  e_0(a_0,a_1) := \mbe_0[e^{-\ka_0(a_0,a_1)} | \la_{\ta^*} \leq -a_0 ] \,. 
            \end{align}    
            Then we can relate the thresholds to the error rates (without the no-overshoots approximation, \citeApp{tartakovsky1991sequential}):
            \begin{equation}
                \al_0^* = \f{
                    e_1(a_0,a_1) e^{a_0} - e_1(a_0,a_1) e_0(a_0,a_1)
                }{
                    e^{a_1+a_0} - e_1(a_0,a_1) e_0(a_0,a_1)
                }, \,\,\, \al_1^* = \f{
                    e_0(a_0,a_1) e^{a_1} - e_1(a_0,a_1) e_0(a_0,a_1)
                }{
                    e^{a_1+a_0} - e_1(a_0,a_1) e_0(a_0,a_1)
                } \,.
            \end{equation}
            To obtain more specific dependence on the thresholds $a_y$ ($y\in\{1,0\}$), we adopt the asymptotic approximation. Let $T_0(a_0)$ and $T_1(a_1)$ be the one-sided stopping times, i.e., $T_0(a_0) := \mr{inf}\{T\geq 1 | \la_T \leq -a_0 \}$ and $T_1(a_1) := \mr{inf} \{T\geq 1 | \la_T \geq a_1 \}$. We then define the associated overshoots as 
            \begin{align}
                &\ti{\ka}_1 (a_1) := \la_{T_1} - a_1 \quad \textrm{on} \{T_1<\infty\} \, , \\    
                &\ti{\ka}_0 (a_0) := -(\la_{T_0} + a_0) \quad \textrm{on} \{T_0<\infty\}\, .
            \end{align}
            According to \citeApp{lotov1988asymptotic}, we can show that 
            \begin{equation}
                \al_0^* \approx \f{
                    \ze_1 e^{a_0} - \ze_1 \ze_0
                }{
                    e^{a_0+a_1} - \ze_1\ze_0
                }, \,\,\, \al_1^* \approx \f{
                    \ze_0 e^{a_1} - \ze_1 \ze_0
                }{
                    e^{a_0+a_1} - \ze_1\ze_0
                } 
            \end{equation}
            under the asymptotic approximation. Note that
            \begin{equation}
                \ze_y := \lim_{a_y\rightarrow\infty}\mbe_y[e^{-\ti{\ka}_y}] \quad (y\in\{1,0\}) \label{eq:zeta}
            \end{equation}                        
            have no dependence on the thresholds $a_y$ ($y\in\{1,0\}$). Therefore we have obtained more precise dependence of the error rates on the thresholds than (\ref{eq:asymptotic}):
            \begin{theorem}{\bf The Asymptotic tradeoff with overshoots}
                Assume that $0<I_y<\infty$ ($y\in\{1,0\}$). Let $\ze_y$ be given in (\ref{eq:zeta}). Then
                \begin{equation}
                    \al_0^* = \ze_1 e^{-a_1}(1+o(1)), \quad \al_1^* = \ze_0 e^{-a_0}(1 + o(1)) \quad (a_0, a_1 \longrightarrow \infty) \, .
                \end{equation}
            \end{theorem}

        \paragraph{Mean hitting time with overshoots.}A more general form of the mean hitting time is provided in \citeApp{tartakovsky1991sequential}. We can show that 
            \begin{align}
                &\mbe_1\ta^* = \f{1}{I_1} \bigg[ \Big(1-\al_1^*\Big) \Big(a_1 + \mbe_1[\ka_1|\ta^*=T]\Big) - \al_1^*\Big(a_0 + \mbe_1[\ka_0|\ta^*=T_0]\Big) \bigg] \label{mean_hitting_time_ov1}\\
                &\mbe_0\ta^* = \f{1}{I_0} \bigg[ \Big(1-\al_0^*\Big) \Big(a_0 + \mbe_0[\ka_0|\ta^*=T]\Big) - \al_0^*\Big(a_1 + \mbe_0[\ka_1|\ta^*=T_1]\Big) \bigg] \, .\label{mean_hitting_time_ov0}
            \end{align}
            The mean hitting times (\ref{mean_hitting_time_ov1}-\ref{mean_hitting_time_ov0}) explicitly depend on the overshoots, compared with (\ref{eq:mean_hitting_time_no_overshoot1}-\ref{eq:mean_hitting_time_no_overshoot0}). Let
            \begin{equation}
                \ch_y := \lim_{a_th\rightarrow\infty}\mbe_y[\ti{\ka}_y] \quad (y \in \{1,0\})
            \end{equation}
            be the limiting average overshoots in the one-sided tests. Note that $\ch_y$ have no dependence on $a_y$ ($y\in\{1,0\}$). The asymptotic mean hitting times with overshoots are
            \begin{equation}
                \mbe_1\ta^* = \f{1}{I_1} (a_1 + \ch_1) + o(1), \quad \mbe_0\ta^* = \f{1}{I_0}(a_0 + \ch_0) + o(1) \quad (a_0 e^{-a_1} \rightarrow0, \quad 
                a_1 e^{-a_0} \rightarrow 0 )\,
            \end{equation}
            As expressed in \citeApp{TartarBook}. Therefore, they have an asymptotically linear dependence on the thresholds.

    \subsection{The Neyman-Pearson Test and SPRT}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    So far, we have discussed the tradeoff of the false alarm rate and the mean hitting time and several properties of the operation characteristic and the mean hitting time. Next, we compare SPRT with the Neyman-Pearson test, which is well-known to be optimal in the \textit{classification} of time-series with \textit{fixed} sample lengths; in contrast, SPRT is optimal in the \textit{early classification} of time-series with \textit{indefinite} sample lengths, as we show in the next section. 
    
    We show that the Neyman-Pearson test is optimal in the two-hypothesis testing problem or the binary classification of time-series. Nevertheless, we show that in the i.i.d. Gaussian model, SPRT terminates earlier than the Neyman-Pearson test despite the same error rates. 
    
    \paragraph{Preliminaries.}Before defining the Neyman-Pearson test, we specify what the "best" test should be. There are three criteria, namely the most powerful test, Bayes test, and minimax test. To explain them in detail, we have to define the size and the power of the test. The significance level, or simply the size of test $d$ is defined as\footnote{
            $P(d=1|y=0)$ is short for $P(\{\om\in\Om|d(X^{(1,T)}) (\om) = 1  \}|y=0)$ and is equivalent to $\mbp_{X^{(1,T)}\sim p(X^{(1,T)}|y=1)} [ d(X^{(1,T)}) = 1 ]$ (i.e., the probability of the decision being 1, where $X^{(1,T)}$ is sampled from the density $p(X^{(1,T)}|y=1)$ ).}
        \begin{equation}
            \al := P(d=1|y=0)\, .
        \end{equation}
        It is also known as the false positive rate, the false alarm rate, or the false acceptance rate of the test. On the other hand, the power of the test $d$ is given by
        \begin{equation}
            \ga := 1-\be := P(d=1|y=1) \,.
        \end{equation}
        $\ga$ is also called the true positive rate, the true acceptance rate. the recall, or the sensitivity. $\be$ is known as the false negative rate or the false rejection rate. 
        
        Now, we can define the three criteria mentioned above.
        \begin{definition}{\bf Most powerful test}\mbox{}\\
            The most powerful test $d$ of significance level $\al(>0)$ is defined as the test that for every other test $d^\prime$ of significance level $\al$, the power of $d$ is greater than or equal to that of $d^\prime$:
            \begin{equation}
                P(d=1|y=1) \geq P(d^\prime=1|y=1) \, .
            \end{equation}
        \end{definition}
        \begin{definition}{\bf Bayes test}\mbox{}\\
            Let $\pi_0 := P(y=0)$ and $\pi_1:= P(y=1) = 1-\pi_0$ be the prior probabilities of hypotheses $H_0$ and $H_1$, and $\bar{\al}(d)$ be the average probability of error:
            \begin{equation}
                \bar{\al}(d) := \sum_{i=1,0} \pi_i \al_i(d) \, ,
            \end{equation}
            where $\al_i(d) := P(d\neq i|y=i)$ is the false negative rate of the class $i\in\{1,0\}$.
            A Bayes test, denoted by $d^{\rm B}$, for the priors is defined as the test that minimizes the average probability of error:
            \begin{equation}
                d^{\rm B} := \underset{d}{\mr{arginf}} \{\bar{\al}(d)\} \, ,
            \end{equation}
            where the infimum is taken over all fixed-sample-size decision rules.
        \end{definition}
        \begin{definition}{\bf Minimax test}\mbox{}\\
            Let $\al_{\rm max}(d)$ be the maximum error probability:
            \begin{equation}
                \al_{\rm max}(d) := \underset{i\in\{1,0\}}{\rm max}\{\al_i(d)\} \, .
            \end{equation}
            A minimax test, denoted by $d^{\rm M}$, is defined as the test that minimizes the maximum error probability:
            \begin{equation}
                \al_{\rm max}(d^{\rm M}) = \underset{d}{\mr{inf}} \{ \al_{\rm max}(d) \} \, ,
            \end{equation}
            where the infimum is taken over all fixed-sample-size tests.
        \end{definition}
        Note that a \textit{fixed-sample-size decision rule} or \textit{non-sequential rule} is the decision rule with a fixed stopping time $T=N$ with probability one. 
    
    \paragraph{Definition and the optimality of the Neyman-Pearson test.}Based on the above notions, we state the definition and the optimality of the Neyman-Pearson test. We see the most powerful test for the two-hypothesis testing problem is the Neyman-Pearson test; the theorem below is also the definition of the Neyman-Pearson test.
        \begin{theorem}{\bf Neyman-Pearson lemma}
            Consider the two-hypothesis testing problem, i.e., the problem of testing two hypotheses $H_o: P=P_0$ and $H_1:P_1$, where $P_0$ and $P_1$ are two probability distributions with densities $p_0$ and $p_1$ with respect to some probability measure. The most powerful test is given by
            \begin{eqnarray}
                d^{\rm NP}(X^{(1,T)}) :=
                \begin{cases}
                    1 & \textrm{if $\La(X^{(1,T)}) \geq h(\al)$} \\
                    0 & \textrm{otherwise}\, ,
                \end{cases}
            \end{eqnarray}
            where $\La(X^{(1,T)})=\f{p_1(X^{(1,T)})}{p_0(X^{(1,T)})}$ is the likelihood ratio and the threshold $h(\al)$ is defined as 
            \begin{equation}
                \al_0(d^{\rm NP}) \bigg(\equiv P(d^{\rm NP}(X^{(1,T)})=1|H_0) =\mbe_0[d^{\rm NP}(X^{(1,T)})]\bigg) = \al 
            \end{equation}
            to ensure for the false positive rate to be the user-defined value $\al(>0)$.
        \end{theorem}
        $d^{\rm NP}$ is referred to as the Neyman-Pearson test and is also optimal with respect to the Bayes and minimax criteria:
        \begin{theorem}{\bf Neyman-Pearson test is Bayes optimal}
            Consider the two-hypothesis testing problem. Given a prior distribution $\pi_i$ ($i\in\{1,0\}$) the Bayes test $d^{\rm B}$, which minimizes the average error probability $\bar{\al}(d) = \pi_0\al_0(d) + \pi_1\al_1(d)$, is given by
            \begin{eqnarray}
                d^{\rm B}(X^{(1,T)}) =
                \begin{cases}
                    1 & (\textrm{if $\La(X^{(1,T)})\geq \pi_0/\pi_1$})\\
                    0 & (\textrm{otherwise}) \, .
                \end{cases}
            \end{eqnarray}
            That is, the Bayesian test is given by the Neyman-Pearson test with the threshold $\pi_0/\pi_1$.
        \end{theorem}
        \begin{theorem}{\bf Neyman-Pearson test is minimax optimal}
            Consider the two-hypothesis testing problem. the minimax test $d^{\rm M}$, which minimizes the maximal error probability $\al_{\rm max}(d) = \underset{i\in\{1,0\}}{\rm max}\{ \al_i(d) \}$, is the Neyman-Pearson test with the threshold such that $\al_0(d^{\rm M}) = \al_1(d^{\rm M})$.
        \end{theorem}
        The proofs are given in \citeApp{borovkov1998mathematical} and \citeApp{lehmann2006testing}.
            
    \paragraph{The SPRT is more efficient.}We have shown that the Neyman-Pearson test is optimal in the two-hypothesis testing problem, in the sense that the Neyman-Pearson test is the most powerful, Bayes, and minimax test; nevertheless, we can show that SPRT terminates faster than the Neyman-Pearson test even when these two show the same error rate.
        
        Consider the two-hypothesis testing problem for the i.i.d. Gaussian model:
        \begin{eqnarray}
            \begin{cases}
                & H_i: y=y_i \quad (i\in\{1,0\})\\
                & x^{(t)} = y + \xi^{(t)} \quad (t \geq 1, y \in \mbr^1)\\
                & \xi^{(t)} \sim \mathcal{N}(0,\si^2) \quad (\si \geq 0)\,,
            \end{cases}
        \end{eqnarray}
        where $\mathcal{N}(0,\si^2)$ denotes the Gaussian distribution with mean 0 and variance $\si^2$. The Neyman-Pearson test has the form
        \begin{eqnarray}
            d^{\rm NP}(X^{(1, n(\al_0,\al_1))}) =
            \begin{cases}
                & 1 \quad (\textrm{if $\la_{n(\al_0,\al_1)} \geq h(\al_0,\al_1)$})\\
                & 0 \quad (\textrm{otherwise}) \,.
            \end{cases}
        \end{eqnarray}
        The sequence length $n=n(\al_0,\al_1)$ and the threshold $h = h(\al_0,\al_1)$ are defined so as for the false positie rate and the false negative rate to be equal to $\al_0$ and $\al_1$ respectively; i.e., 
        \begin{align}
            P(\la_n \geq h| y=y_0) = \al_0 \, ,\\
            P(\la_n < h| y=y_1) = \al_1 \,.
        \end{align}
        We can solve them for the i.i.d. Gaussian model (\citeApp{TartarBook}). To see the efficiency of SPRT to the Neyman-Pearson test, we define
        \begin{align}
            \mce_0 (\al_0, \al_1) = \f{\mbe [\ta^*|y=y_0]}{n(\al_0,\al_1)} \\
            \mce_1 (\al_0, \al_1) = \f{\mbe [\ta*|y=y_1]}{n(\al_0,\al_1)} \,.
        \end{align}
        Assuming the overshoots are negligible, we obtain the following asymptotic efficiency (\citeApp{TartarBook}):
        \begin{equation}
            \lim_{\mr{max\{ \al_0,\al_1 \} \rightarrow 0}} \mce_y (\al_0,\al_1) = \frac{1}{4} \quad (y \in \{1,0\}) \,.
        \end{equation}
        In other words, under the no-overshoot and the asymptotic assumptions, SPRT terminates four times earlier than the Neyman-Pearson test in expectation, despite the same false positive and negative rates.
        
    \subsection{The Optimality of SPRT}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    \paragraph{Optimality in i.i.d. cases.}\label{app:optimality_detail}
    The theorem below shows that SPRT minimizes the expected hitting times in the class of decision rules that have bounded false positive and negative rates. Consider the two-hypothesis testing problem. We define the class of decision rules as
        \begin{equation}\label{eq:i.i.d. termination}
            C(\al_0, \al_1) = \{
                \de \quad \mr{s.t.} \quad P(d=1|H_0) \leq \al_0, P(d=0|H_1) \leq \al_1, \mbe[\ta|H_0] < \infty, \mbe[\ta|H_1] < \infty
            \} \,.
        \end{equation}
         Then the optimality theorem states:
        \begin{theorem}{\bf I.I.D. Optimality (\citeApp{TartarBook})} \label{thm:iid optimality}
            Let the time-series data points $x^{(t)}$, $t=1,2,...$ be i.i.d. with density $f_0$ under $H_0$ and with density $f_1$ under $H_1$, where $f_0 \not\equiv f_1$. Let $\al_0 > 0$ and $\al_1>0$ be fixed constants such that $\al_0 + \al_1 <1$. If the thresholds $-a_o$ and $a_1$ satisfies $\al_0^*(a_0, a_1) = \al_0$ and $\al_1^*(a_0, a_1) = \al_1$, then SPRT $\de^* = (d^*, \ta^*)$ satisfies
            \begin{equation}
                \underset{\de = (d,\ta)\in C(\al_0,\al_1)}{\rm inf}\bigg\{\mbe[\ta|H_0]\bigg\} = \mbe[\ta^*|H_0] 
                \quad \textrm{and} \quad
                \underset{\de = (d,\ta)\in C(\al_0,\al_1)}{\rm inf}\bigg\{\mbe[\ta|H_1]\bigg\} = \mbe[\ta^*|H_1]
            \end{equation}
        \end{theorem}
        A similar optimality holds for continuous-time processes (\citeApp{irle1984optimality}). Therefore SPRT terminates at the earliest stopping time in expectation of any other decision rules achieving the same or less error rates --- SPRT is optimal.
        
        Theorem \ref{thm:iid optimality} tells us that given user-defined thresholds, SPRT attains the optimal mean hitting time. Also, remember that the thresholds determine the error rates (e.g., Equation (\ref{eq:asymptotic})). Therefore, SPRT can minimize the required number of samples and achieve the desired upper-bounds of false positive and false negative rates.

    %\paragraph{Optimal Truncated Test}
    
    %\paragraph{KL-Optimality in the Non-I.I.D. Case}
    
    \paragraph{Asymptotic optimality in general non-i.i.d. cases.}In most of the discussion above, we have assumed the time-series samples are i.i.d. For general non-i.i.d. distributions, we have the asymptotic optimality; i.e., SPRT asymptotically minimizes the moments of the stopping time distribution (\citeApp{TartarBook}).
        
        Before stating the theorem, we first define a type of convergence of random variables.
        \begin{definition}{\bf r-quick convergence}
            Let $\{ x^{(t)} \}_{t\geq 1}$ be a stochastic process. Let $\mathcal{T}_\ep(\{ x^{(t)} \}_{t\geq 1})$ be the last entry time of the stochastic process $\{ x^{(t)} \}_{t\geq 1}$ in the region $(\ep, \infty) \cup (-\infty, -\ep)$, i.e.,
            \begin{equation}
                \mathcal{T}_\ep(\{ x^{(t)} \}_{t\geq 1}) = \underset{t\geq 1}{\rm sup}\{ t \,\,\,\textrm{s.t.}\,\,\, |x^{(t)}|>\ep \}, \quad \mr{sup}\{\emptyset\} := 0 \,.
            \end{equation}
            Then, we say that the stochastic process $\{ x^{(t)} \}_{t\geq 1}$ converges to zero r-quickly, or 
            \begin{equation}
                x^{(t)} \underset{t\rightarrow \infty}{\xrightarrow{r-{\rm quickly}}} 0 \, ,
            \end{equation}
            for some $r>0$, if
            \begin{equation}
                \mbe[(\mathcal{T}_\ep(\{ x^{(t)} \}_{t\geq 1}))^r] < \infty \quad \textrm{for every $\ep>0$}\,.
            \end{equation}
        \end{definition}
        $r$-quick convergence ensures that the last entry time in the large-deviation region ($\mathcal{T}_\ep(\{ x^{(t)} \}_{t\geq 1})$) is finite almost surely. The asymptotic optimality theorem is:
        \begin{theorem}{\bf Non-i.i.d. asymptotic optimality} \label{thm:non-iid optimality}
            If there exist positive constants $I_0$ and $I_1$ and an increasing non-negative function $\ps(t)$ such that
            \begin{equation}\label{eq:non-i.i.d. termination}
                \f{\la_t}{\ps(t)} \underset{t\rightarrow \infty}{\xrightarrow{P_1-r-{\rm quickly}}} I_1 \quad\textrm{and}\quad 
                \f{\la_t}{\ps(t)}\underset{t\rightarrow \infty}{\xrightarrow{P_0-r-{\rm quickly}}} -I_0 \, ,
            \end{equation}
            where $\la_t$ is defined in section \ref{sec:preliminaries}, then
            \begin{equation}
                \mbe[(\ta^*)^r | y=i] < \infty \quad \textrm{($i \in \{1,0\}$) for any finite $a_0$ and $a_1$}.
            \end{equation}
            Moreover, if the thresholds $a_0$ and $a_1$ are chosen to satisfy (\ref{eq:exact}), $a_0\rightarrow\log (1/\al_1^*)$, and $a_1\rightarrow\log (1/\al_0^*)$ ($a_i \rightarrow\infty$), then for all $0<m\leq r$,
            \begin{align}
                & \underset{\de\in C(\al_0,\al_1)}{\rm inf}\left\{ \mbe[\ta^m | y=y_1]\right\} - \mbe[(\ta^*)^m | y=y_1] \longrightarrow 0 \\
                & \underset{\de\in C(\al_0,\al_1)}{\rm inf}\left\{ \mbe[\ta^m | y=y_0]\right\} - \mbe[(\ta^*)^m | y=y_0] \longrightarrow 0 
            \end{align}
            as $\mr{max}\{ \al_0, \al_1 \} \longrightarrow 0$ with $| \log\al_0 / \log\al_1 | \longrightarrow c$, where $c\in (0,\infty)$.
        \end{theorem}









    
\newpage










